Turbulent Drag Reduction in Magnetohydrodynamic Turbulence and Dynamo from Energy Flux Perspectives

In this review, we describe turbulent drag reduction in a variety of flows using a universal framework of energy flux. In a turbulent flow with dilute polymers and magnetic field, the kinetic energy injected at large scales cascades to the velocity field at intermediate scales, as well as to the polymers and magnetic field at all scales. Consequently, the kinetic energy flux, $ \Pi_u(k) $, is suppressed in comparison to the pure hydrodynamic turbulence. We argue that the suppression of $\Pi_u(k)$ is an important factor in the reduction of the inertial force $\langle {\bf u \cdot \nabla u} \rangle$ and \textit{turbulent drag}. This feature of turbulent drag reduction is observed in polymeric, magnetohydrodynamic, quasi-static magnetohydrodynamic, and stably-stratified turbulence, and in dynamos. In addition, it is shown that turbulent drag reduction in thermal convection is due to the smooth thermal plates, similar to the turbulent drag reduction over bluff bodies. In all these flows, turbulent drag reduction often leads to a strong large-scale velocity in the flow.

==> dns_old.tex <==


\section{Numerical verification of TDR  in MHD turbulence }
\label{sec:dns}

Many researchers have simulated MHD turbulence, but drag reduction in MHD turbulence has not been explored in detail.  In this section, we will discuss this issue from the perspectives of numerical results from direct numerical simulations (DNS) and shell models.

MHD turbulence exhibits six energy fluxes that are shown in Fig.~\ref{fig:mhd_fluxes}.  These fluxes represent energy transfers from $ u^< $ and $ u^> $ to $ b^< $ and $ b^> $. 
However, as we discussed in Sec.~\ref{sec:drag}, the relevant fluxes for turbulent drag reduction are $ \Pi_u $ and $ \Pi_B $. Also, the turbulent drag reduction takes place at large scales, hence, these fluxes originate from small $ k_0 $.  In terms of the fluxes of Fig.~\ref{fig:mhd_fluxes},
\bea
\Pi_u(k_0) & = & \Pi^{u<}_{u>}(k_0) \\
\Pi_B(k_0) & =  & \Pi^{u<}_{b<}(k_0) +  \Pi^{u<}_{b>}(k_0)
\eea
 Here, we will show that $ \Pi_B > 0 $, and hence, according Eq.~(\ref{eq:Pi_tot}), $ \Pi_u  < \epsilon_\mathrm{inj}$.  Therefore, $ \Pi_u $ is suppressed compared to hydrodynamic turbulence.  In this section, we will verify the above inequality, as well as compare  $\la \lvert ({\bf u}\cdot \nabla) {\bf u} \rvert  \ra$ for  HD and MHD turbulence.
\begin{figure}%[tbhp]
	\centering
	\includegraphics[scale=0.7]{fig/mhd_fluxes.pdf}
	\caption{Six energy fluxes of MHD turbulence: $ \Pi^{u<}_{u>} $, $ \Pi^{u<}_{b<} $, $ \Pi^{u<}_{b>} $, $ \Pi^{b<}_{b>} $, $ \Pi^{b<}_{u>} $, $ \Pi^{u>}_{b>} $. From Verma~\cite{Verma:book:ET}.  Reproduced with permission from Verma.}
	\label{fig:mhd_fluxes}
\end{figure}
 
It is important to note that the velocity field receives parts of  $ \Pi_B $   via the energy fluxes $ \Pi^{b<}_{u>} $ and $ \Pi^{b>}_{u>}  $. However, these transfers are effective at large wavenumbers. In this review we focus on small wavenumbers, hence we can ignore these energy transfers.  In the following discussion, we will compute $ \Pi_B $ using  numerical simulations and shell model.
%%%%

\subsection{Turbulence drag reduction in direct numerical simulation of MHD turbulence}
We solve the nondimensional MHD equations~(\ref{eq:U_MHD}-\ref{eq:b_incompress}) using pseudo-spectral code TARANG~\cite{Boyd:book:Plasma,Verma:Pramana2013tarang,Chatterjee:JPDC2018} in a cubic periodic box with a box-size of $(2\pi)^3$.   We nondimensionalize  velocity, length, and  time  using the initial rms speed ($U_0$), box size $ (2\pi) $, and the eddy turnover time ($2\pi / U_0)$, respectively. We  employ the fourth-order Runge-Kutta scheme for time marching; Courant-Friedrich-Lewis (CFL) condition for computing the time  step $\Delta t$; and  $2/3$ rule for dealising. We  perform our simulations on a $256^3$ grid  for  $ \mathrm{Pm}=1.3, 1, 10/3 $ (the details in the following discussion).  The mean magnetic field in our simulation is zero, i.e., ${\bf B}_0 = 0$.   Note that the $ 256^3 $ grid resolution is sufficient for estimating large-scale $ \Pi_u, \Pi_B $, and nonlinearity.  In addition, the low resolution helps us run the simulations for a long time.

For the initial condition, we employ random velocity and magnetic fields at all wavenumber.  For creating such fields, it is convenient to employ Craya-Herring basis~\cite{Craya:thesis, Herring:PF1974}, whose  basis vectors for wavenumber $ {\bf k} $ are
\begin{equation}
	\hat{\bf e}_3(\mathbf{k}) = \hat{\bf k};~~~\hat{\bf e}_1(\mathbf{k}) =  ( \hat{\bf k} \times \hat{\bf n})/ \lvert \hat{\bf k} \times \hat{\bf n}\rvert;~~~ \hat{\bf e}_2(\mathbf{k}) = \hat{\bf k} \times \hat{\bf e}_1(\mathbf{k}), 
\end{equation}
where $\hat{\bf n}$ is chosen along any arbitrary direction, and $\hat{\bf k}$ is the unit vector along  $\mathbf{k}$. We choose 3D incompressible flow, hence,
\begin{equation}
	\mathbf{u}(\mathbf{k}) = u_1(\mathbf{k}) \hat{\bf e}_1(\mathbf{k}) + u_2(\mathbf{k}) \hat{\bf e}_2(\mathbf{k}).
\end{equation}
For random initial velocity with the total kinetic energy as $ E_u $, we employ
\begin{eqnarray}
	u_1(\mathbf{k}) & = & \sqrt{(E_u/2N^3)} \ i \left(\exp(i \phi_1(\mathbf{k})) - \exp(i \phi_2(\mathbf{k})) \right), \\
	u_2(\mathbf{k}) & = & \sqrt{(E_u/2N^3)} \ \left(\exp(i \phi_1(\mathbf{k})) + \exp(i \phi_2(\mathbf{k}))\right),
\end{eqnarray}
where $N^3$ is the total number of modes, and the phases $\phi_1(\mathbf{k})$ and $\phi_2(\mathbf{k})$ are chosen randomly from uniform distribution in the band $[0, 2\pi]$.  We employ $ E_u=0.5 $ for our simulation. A similar scheme is adopted for the random magnetic field with the   initial magnetic energy as 0.25.  We carry out the above run for $ \nu = 10^{-2} $, $ \eta = 10^{-2} $, or $ \mathrm{Pm}=1$.


We  force  the velocity modes in a wavenumber shell $(2,3)$, denoted by $k_f = 2$, randomly so as to  achieve a steady state~\cite{Sadhukhan:PRF2019}.  The kinetic-energy injection rate $ \epsilon_\mathrm{inj}  = 0.4$. We carry out the MHD turbulence simulation till 29 eddy turnover time. Note, however, that the flow reaches a steady state in approximately $15$ eddy turnover time. 

At  the end of the above simulation, we perform the following four runs:
\begin{enumerate}
	\item MHD1:  $ \nu = 0.01 $, $ \eta = 0.03$, and hence $ \mathrm{Pm}=1/3 $.

\item MHD2:   $ \nu = 0.01 $, $ \eta = 0.03$, and hence $ \mathrm{Pm}=1$. This is continuation of the preliminary run.

\item MHD3:  $ \nu = 0.01 $, $ \eta = 0.003$, and hence $ \mathrm{Pm}=1/3 $.

\item HD: $ \nu = 0.01$ with magnetic field turned off.
\end{enumerate}
For the subsequent description, we treat this as the initial state  ($ t=0 $), and carry forward the HD and MHD2 simulations  till 40 eddy turnover times, while MHD1 and MHD3 runs till 5 eddy turnover times.  Subsequently we will compare the energy fluxes and $\la \lvert ({\bf u}\cdot \nabla) {\bf u} \rvert  \ra$ of all the four runs after they have reached their respective steady states (in several eddy turnover times). Under the steady state of HD run, the Reynolds numbers ($ \mathrm{Re} = UL/\nu $) is 457. For the MHD runs with $ \mathrm{Pm}=1/3, 1, $ and 10/3,  $ \mathrm{Re} = xxx $ respectively, while $ \mathrm{Rm} = xxx $ respectively.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}%[tbhp]
	\centering
	\includegraphics[scale=0.6]{fig/Figure7.pdf}
	\caption{Left column: (a,c,e) Time series of KE of HD turbulence (dashed red curve), KE  (solid red curve), magnetic energy (solid green curve) and total energy (solid blue curve) of MHD turbulence for $ \mathrm{Pm}=1/3, 1, 10/3 $. Right column: (b,d,f) Corresponding energy dissipation rates with the same notation.}
	\label{fig:dns_energy_evolution}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\begin{table}[h]
%		\begin{minipage}{\textwidth}
%			\caption{Simulation parameters: Grid resolution ($N$), energy injection rate ($\epsilon_{\rm{inj}}$), kinematic viscosity ($\nu$), magnetic diffusivity ($\eta$), Magnetic Prandtl number ($\mathrm {Pm}$), kinetic Reynolds number for hydrodynamic ($\mathrm {Re}_{\rm {HD}} = U L_b/ \nu$), kinetic Reynolds number for MHD ($\mathrm {Re}_{\rm {MHD}} = U L_b / \nu$) and magnetic Reynolds number ($\mathrm {Rm} = U L_b / \eta$), where $L_b = 2\pi$ is the box size. The parameters are averaged in time domain $t \in [20,40]$.} \label{tab:table1_dns}%
%			\vspace{10pt}%
%			\begin{center}
%			\begin{tabular}{@{}llllllll@{}}
%				\toprule
%				{$N$}	& $\epsilon_{\rm {inj}}$ & $\nu$ & $\eta$ & $\rm{Pm}$ & $\rm{Re}_{\rm {HD}}$ & {$\rm{Re}_{\rm {MHD}}$} & {${\rm {Rm}}$}\\
%				\midrule
%				$256^3$		& $0.4$	 & $0.01$& $0.01$ & $1$       & $457 $               &$ 348$ & $348$\\
%				\botrule
%			\end{tabular}
%		\end{center}
%		\end{minipage}
%\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


In Fig.~\ref{fig:dns_energy_evolution}(left column), we show the time  series of KE (dashed red curve) of HD turbulence, and as well as KE (solid red curve), ME (solid green curve), and the total energy (solid blue curve) of MHD turbulence for the three runs. The corresponding dissipation rates are exhibited in the right column of Fig.~\ref{fig:dns_energy_evolution}.  As shown in the figures, both the systems reach steady states after several eddy turnover time. The KE dissipation rate for the HD turbulence increases rapidly to the KE injection rate ($\epsilon_{\rm {inj}}$) of 0.4, whereas the kinetic energies for the MHD turbulence  with  $ \mathrm{Pm} =  $ saturate respectively to approximate values of XXX . Note that energies for MHD turbulence  exhibit significant fluctuations, however, the dissipation rate of the total energy remains at 0.4. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\begin{figure}[tbhp]
	\centering
	\includegraphics[scale = 0.7]{fig/Figure8.pdf}
	\caption{(a,b,c) For $ \mathrm{Pm} = 1/3, 1, 10/3 $, plots of the KE spectra of HD (dashed red curve) and MHD turbulence (solid red curve). The magnetic energy spectra (solid green curve) for MHD turbulence are also shown. }
	\label{fig:spectrum_comp_dns}
\end{figure}

Now, we report the  energy spectra for the velocity and magnetic fields for a wavenumber $ k $. Numerically, we compute them using
\begin{eqnarray}
	E_u(k) &=& \frac{1}{2} \sum_{k-1 < \lvert \mathbf {k'} \rvert \leq k} \lvert \bf{u}(\bf {k'}) \rvert^2, \label{eq:dns_ke} \\
	E_b(k) &=& \frac{1}{2} \sum_{k-1 < \lvert \mathbf {k'} \rvert \leq k} \lvert \bf{b}(\bf {k'}) \rvert^2 \label{eq:dns_me}, 
\end{eqnarray}
In Fig.~\ref{fig:spectrum_comp_dns}, we exhibit $ E_u(k), E_b(k) $ for MHD turbulence. These quantities are averaged  over $2000$  time frames between the time interval $(20,40)$.  In the same figure, we also exhibit $ E_u(k)$ for the HD turbulence.  We observe that  $ E_u(k) $ for HD turbulence is larger than those for MHD turbulence, except at low wavenumbers for $ \mathrm{Pm}=1/3 $ where $ E_b(k) > E_u(k) $.

Further, for both HD and MHD turbulence, we report the rms speeds $U$, integral length scales $L$, and Reynolds numbers based on  Taylor microscale, $\mathrm {Re}_{\lambda} = U \lambda/\nu$, where Taylor microscale $\lambda = (15 \nu U^2/\epsilon)^{1/2}$~\cite{Lesieur:book:Turbulence}. Here, $ U $  represents the rms value for each component of the velocity~\cite{Sreenivasan:PF1998}:
\be
U = \left[ \frac{2}{3} \int dk E(k) \right]^{1/2},
\ee
whereas  the integral length $ L $ is defined using
\be
L = \frac{\int dk k^{-1} E(k)}{\int dk E(k)}.
\ee
\begin{figure}[tbhp]
	\centering
	\includegraphics[width=\linewidth]{fig/Figure9.pdf}
	\caption{Time evolution of rms velocity ($U$), $ U(K=1) $, $ U(K=2) $, integral length scale ($L$), and (c)  Reynolds number based on Taylor microscale ($\mathrm{Re}_{\lambda}$) for HD (dashed red curve) and MHD turbulence (solid red curve) for $ \mathrm{Pm}=1/3, 1, 10/3 $. $ U(K=1) $ and $ U(K=2) $ computed using the kinetic energy contained in waveumber spheres of radii 1 and 2 respectively. }
	\label{fig:time_evol_dns}
\end{figure}

\begin{table}[h]
	\begin{minipage}{\textwidth}
		\caption{For $\epsilon_\mathrm{inj}=0.4$, Numerical values of average KE flux ($\la \Pi_{u} \ra $) in the inertial range,  rms velocity ($U$), $\langle \lvert (\mathbf{u}\cdot\nabla)\mathbf{u} \rvert \rangle$, $\bar{C}_{d1}$,  and $\bar{C}_{d2}$ for sphere of  radii $K=1$ and $K=2$.  }
		\label{tab:table2_dns}
		\vspace{10pt}
		\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lcccccccccc@{\extracolsep{\fill}}}
			\toprule%
			& & & & & \multicolumn{2}{@{}c@{}}{$K=1$} & \multicolumn{2}{@{}c@{}}{$K=2$} \\\cmidrule{6-7}\cmidrule{8-9}%
			& $ \mathrm{Pm} $ & $ \la \Pi_{u} \ra $ & $U$ & $\la \bar{C}_{d1} \ra $ &$\la \lvert ({\bf u}\cdot \nabla) {\bf u} \rvert  \ra$ & $\la \bar{C}_{d2} \ra$ & $\la \lvert ({\bf u}\cdot \nabla) {\bf u} \rvert \ra $ & $\la \bar{C}_{d2} \ra$ \\ \\
			\midrule
			\rm{HD} & - &  $0.35$  & $0.72$ & $0.58$  & $0.1$  & $0.13$ & $0.3$  & $0.37$ \\
			\rm{MHD} & $1/3$ & $0.28$ & $0.66$ & $0.65$ & $0.07$ & $0.11$	 & $0.3$ & $0.46$  \\
			\rm{MHD} & $1$ & $0.25$ & $0.55$ & $0.98$ & $0.06$ & $0.13$ & $0.22$ & $0.49$ \\
			\rm{MHD} & $10/3$ & $0.17$ & $0.53$ & $0.8$ & $0.04$ & $0.09$ & $0.17$ & $0.41$\\
			\botrule
		\end{tabular*}
	\end{minipage}
\end{table}


In Fig.~\ref{fig:time_evol_dns}, we exhibit  the time series of $U$, $L$, and the Reynolds number based on Taylor's microscale ($\mathrm {Re}_{\lambda}$) for both the flows. We quantify $ U $ in three ways: $ U_\mathrm{rms} $; and $ U(K=1) $, and $ U(K=2) $, which are computed using the  contents of kinetic energies in wavenumber spheres are radii 1 and 2 respectively. We compute $\mathrm {Re}_{\lambda}$ using $ U_\mathrm{rms}  $. We list $ U_\mathrm{rms}  $ in Table~\ref{tab:table2_dns}.  In MHD turbulence, the  total energy is shared between the velocity and magnetic fields.  Hence, for the same $\epsilon_{\rm {inj}} $, Hence,  $ U_\mathrm{rms} $  for the MHD run is lower than that for HD run.  However,  for $ \mathrm{Pm} =1 $, $ U(K=1) $ for MHD turbulence is comparable to the that for HD turbulence.  Note that we enlist the above quantities of MHD turbulence for $\mathrm{Pm} = 1/3, 1$ and $10/3$. For $\mathrm{Pm} = 1$, we average the quantities of Table~\ref{tab:table2_dns} over time frames in the time interval $t = [20,40]$ , whereas for $\mathrm{Pm} =1/3$ and $10/3$, averaging was performed in the time interval $t=[3, 5]$. 

As shown in Fig.~\ref{fig:time_evol_dns}, the integral length for the MHD turbulence is larger than the corresponding $ L $ for the HD turbulence. Hence, we conclude that the field variables are more ordered in MHD turbulence than in HD turbulence.  We compute $\mathrm {Re}_{\lambda} = U_\mathrm{rms} L/\nu$ for all the runs.  We observe that for $ \mathrm{Pm} =1/3$, $\mathrm {Re}_{\lambda} $ for MHD turbulence is close to that for HD turbulence, but for the other two magnetic Prandtl numbers, $\mathrm {Re}_{\lambda} $ for MHD turbulence is lower than that for HD turbulence. 


Next, we compute the kinetic energy fluxes, $\Pi_u(K)$, for the HD and MHD turbulence, as well $ \Pi_B(K) $ for the MHD turbulence.  These fluxes exhibit significant fluctuations, hence we average over  several time frames in the steady state.  The fluxes, shown in Fig~\ref{fig:flux_dns},  clearly show that $ \Pi_B > 0 $, indicating energy transfers from the velocity field to magnetic field at all scales, and that
\begin{eqnarray}
	\Pi_{u, \mathrm{MHD}} < \Pi_{u, \mathrm{HD}}.
\end{eqnarray}
\begin{figure}[tbhp]
	\centering
	\includegraphics[scale = 0.6]{fig/Figure10.pdf}
	\caption{(a,b,c) For $ \mathrm{Pm} = 1/3, 1, 10/3 $, plots of $ \Pi_u(K) $ of HD turbulence (dashed red curve); and  $ \Pi_u(K) $  (solid red curve) and  $ \Pi_B(K) $  (solid green curve)  of MHD turbulence.}
	\label{fig:flux_dns}
\end{figure}

Now we compute the drag coefficient $\bar{C}_{d1}$, which is defined in Eq.~(\ref{eq:c1}) as $ \la \Pi_u \ra / (U_\mathrm{rms}^3/L) $ , and exhibit its time series  in Fig.~\ref{fig:dns_drag_c1}. We observe that $\bar{C}_{d1}$ for HD turbulence is consistent with the results of Sreenivasan~\cite{Sreenivasan:PF1998}. In the steady state,  $\bar{C}_{d1}$ of our MHD run is larger than that for HD turbulence for the three MHD runs (see Table~\ref{tab:table2_dns}).  This is because the decrease in $ U $ for the MHD turbulence is stronger than the decrease in $ \Pi_u(K) $. Hence, $ \la \Pi_u \ra / (U^3/L) $ for MHD turbulence is larger than that for HD turbulence. 
\begin{figure}%[tbhp]
	\centering
	\includegraphics[scale=0.6]{fig/Figure11.pdf}
	\caption{(a,b,c) For $ \mathrm{Pm} = 1/3, 1, 10/3 $, time evolution of drag reduction coefficient $\bar{C}_{d1}$ for hydrodynamic turbulence (dashed red curve) and MHD turbulence (solid red curve).}
	\label{fig:dns_drag_c1}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Now, we examine the   nonlinear term $N_u$ of HD  and MHD turbulence. Since the drag force is effective at large scales, we  estimate $N_u$  by  its  rms value for a small  wavenumber sphere  of radius $ K $:
\begin{eqnarray}
	N_{u} & =  \langle \lvert \left(\mathbf{u} \cdot \boldsymbol{\nabla} \right) \mathbf{u} \rvert \rangle_\mathrm{LS}  = & \left( \sum_{k\leq {K}} \lvert \left(\mathbf{k} \cdot \mathbf{u}(\mathbf{k}) \right) \mathbf{u}(\mathbf{k}) \rvert^2 \right)^{\frac{1}{2}}. \label{eq:dns_nonlin} 
\end{eqnarray}
In particular, we choose $K=1$ and $K=2$. In Fig.~\ref{fig:dns_nonlin}(a,b), we illustrate the time series of $N_u$ for HD turbulence (dashed red curve) and MHD turbulence (solid red curve) for $K=1$ and $K=2$.  We observe that $ N_u $ for MHD turbulence is lower than its hydrodynamic counterpart for the three MHD runs. Hence, there is a reduction in nonlinearity for MHD turbulence compared to HD turbulence, signalling turbulent drag reduction.
\begin{figure}[tbhp]
	\centering
	\includegraphics[width=\linewidth]{fig/Figure12.pdf}
	\caption{(a,b,c) For $ \mathrm{Pm} = 1/3, 1, 10/3 $, plots of nonlinear term $(N_u)$ for sphere of radii (a) $K=1$, and (b) $K=2$ of HD turbulence (dashed red curve) and MHD turbulence (solid red curve) vs time.}
	\label{fig:dns_nonlin}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%


After this, we compute the drag reduction coefficient  $\bar{C}_{d2}$, which is defined in Eq.~(\ref{eq:c2}) as $ \la \lvert ({\bf u \cdot \nabla}) {\bf u} \rvert \ra/(U^2/L) $.  The time series of $\bar{C}_{d2}$ for $K=1$ and $K=2$ are plotted in  Figure~\ref{fig:dns_drag_c2}.  We observe that for $ \mathrm{Pm} =1/3 and 10/3 $ and $ K=1 $, 
$\bar{C}_{d2}$ for MHD turbulence is lower than HD turbulence for $ t \gtrapprox 2 $.  However, for other cases, $\bar{C}_{d2}$ for MHD turbulence is marginally larger than that for the HD turbulence. 
\begin{figure}%[tbhp]
	\centering
	\includegraphics[width=\linewidth]{fig/Figure13.pdf}
	\caption{(a,b,c) For $ \mathrm{Pm} = 1/3, 1, 10/3 $, time evolution of drag reduction coefficient $\bar{C}_{d2}$ for sphere of radii (a) $K=1$, and (b) $K=2$ for HD turbulence (dashed red curve) and MHD turbulence (solid red curve).}
	\label{fig:dns_drag_c2}
\end{figure}


Thus, $ \Pi_u $ and $\la \lvert ({\bf u}\cdot \nabla) {\bf u} \rvert  \ra$ for MHD turbulence are lower than  the corresponding values for the HD turbulence for $ 1/3 \le \mathrm{Pm} \le 10/3 $. However, the drag coefficients for MHD turbulence, $\bar{C}_{d1}$ and $\bar{C}_{d2}$, are typically lower than those for HD turbulence, except for some cases with $ \mathrm{Pm} = 1/3  $ and 10/3.
This is because our simulations yield smaller  $ U $ for MHD turbulence  than that for HD turbulence and it overcompensates the decrease in  $ \Pi_u $ and $\la \lvert ({\bf u}\cdot \nabla) {\bf u} \rvert  \ra$.  Note, however, that quasi-static MHD turbulence, which corresponds to $ \mathrm{Pm}=0 $, exhibit increase in $ U $  compared to the respective HD turbulence. Hence, we expect similar behaviour for MHD turbulence with very small $ \mathrm{Pm} $.  This conjecture needs to be tested in future.  In addition, in a channel or in a spherical shell with magnetofluids, $ U $ may be larger when the magnetic field gets turned on.   We will cover some of these aspects in Sec.~\ref{sec:dynamo}.  

After a brief discussion on DNS of MHD turbulence, in the next subsection, we will discuss  turbulent drag reduction  in  the shell model of MHD turbulence.



==> shell_old.tex <==
\subsection{Numerical verification using shell model}
In this subsection we report results of Verma \etal \cite{Verma:PP2020} for a shell model of MHD turbulence. Verma \etal employed a revised version of  Gledzer-Ohkitani-Yamada (GOY) shell model to compute  the drag forces and  nonlinear terms for HD and MHD turbulence~\cite{Gledzer:DANS1973,Yamada:PRE1998,Verma:JoT2016,Verma:PP2020}.  We  show that the turbulent drag  in MHD turbulence is indeed reduced compare to HD turbulence.

In a  shell model of turbulence, all the Fourier modes in a wavenumber shell are represented by a single variable. For $ N $ shells, we have $ N $ velocity and $ N $ magnetic shell variables that are coupled nonlinearly with the neighbouring shells. For more details on  shell models, refer to Ditlevsen \cite{Ditlevsen:book}. In this review we present the results of Verma \etal \cite{Verma:PP2020}. To avoid repetition, we skip the details of the shell model. 
 

Verma \etal \cite{Verma:PP2020}  employed a shell model with $36$  shells, and simulated the  models for HD and MHD turbulence for the same kinetic energy injection rate \cite{Verma:PP2020}.    They   forced the large-scale velocity field using  a random force at shells $n = 1$ and $2$ such that the kinetic energy supply rate is maintained at a constant value~\cite{Stepanov:JoT2006}.   They performed three sets of simulations with  kinetic energy supply rates $\epsilon_\mathrm{inj}=0.1, 1.0$ and $10.0$, and  $\nu =   \eta=10^{-6}$.  For time integration, they used Runge-Kutta fourth order (RK4) scheme with a fixed $\Delta t$. For  $\epsilon_\mathrm{inj}=0.1$ and $1.0$, they chose $\Delta t =5\times10^{-5}$,  but  for $\epsilon_\mathrm{inj}=10.0$, they took $\Delta t =1\times10^{-5}$.  The numerical results are summarized in Table~\ref{tab:HD_MHD_shell}. They carried out the HD and MHD simulations up to  1000 eddy turnover time. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure}%[tbhp]
%	\centering
%	\includegraphics[scale=0.3]{fig/Figure9.pdf}
%	\caption{Time evolution plots of kinetic energy for hydrodynamics; and of kinetic, magnetic, and total energy for MHD turbulence for different injection rates $\epsilon_\mathrm{inj}=0.1$(a),$1.0$(b) and $10.0$(c).  The solid red curve denotes the kinetic energy for hydrodynamic turbulence, and the dashed red, forest green and dark blue curves, respectively, show the kinetic, magnetic and total energy for MHD turbulence.}
%	\label{fig:energy_comp}
%\end{figure}




Both HD and MHD simulations reached their respective steady states after approximately $200$ eddy turnover time.   Interestingly, Verma \etal \cite{Verma:PP2020}  observed  that for the same $\epsilon_\mathrm{inj}$,  the KE and $ U $ for MHD turbulence are larger than those for  HD turbulence, as shown in Table~\ref{tab:HD_MHD_shell}.  These observations clearly demonstrate an enhancement of $ U $ in MHD turbulence compared to HD turbulence, as is the case for flow with dilute polymers.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[h]
	\begin{center}
		\begin{minipage}{\textwidth}
			\caption{For the shell model runs of Verma \etal \cite{Verma:PP2020}, numerical values of inertial-range flux $\Pi_{u}$, rms velocity  $U$, and  $\la  ({\bf u}\cdot \nabla) {\bf u}  \ra=(\sum_{n}N_{n}[u,u]^{2})^{1/2}$ for the injection rates $\epsilon_\mathrm{inj}=0.1,1.0,10.0$ for both HD and MHD runs.} 	\label{tab:HD_MHD_shell}
			\vspace{10pt}
			\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lccccccccccc@{\extracolsep{\fill}}}
				\toprule%
				& \multicolumn{3}{@{}c@{}}{Hydrodynamics} & \multicolumn{3}{@{}c@{}}{MHD} \\\cmidrule{2-4}\cmidrule{5-7}%
				$\epsilon_\mathrm{inj}$ & $\Pi_{u}$ & $U$ & $\la  ({\bf u}\cdot \nabla) {\bf u}  \ra$ &  $ \bar{c}_{d1} $ & $ \bar{c}_{d2} $ & $\Pi_{u}$ & $U$ & $\la  ({\bf u}\cdot \nabla) {\bf u}  \ra$ & $ \bar{c}_{d1} $ & $ \bar{c}_{d2} $ \\
				\midrule
				$0.1$ & $0.1$ & $0.87$ & $8.77$ & $0.02$ & $0.92$ & $4.17$ && \\
				$1.0$ & $1.0$ & $1.88$ & $47.48$ & $0.21$ & $2.02$ & $23.79$  && \\
				$10.0$ & $10.0$ & $3.95$ & $271.88$ & $2.06$ & $4.33$ & $136.44$ && \\
				\botrule
			\end{tabular*}
		\end{minipage}
	\end{center}
\end{table}


The increase in $ U $ for MHD turbulence compared to HD turbulence has its origin in the energy spectra. Verma \etal \cite{Verma:PP2020}  computed the average kinetic energy spectra $  E_u(k) $ for HD and MHD turbulence; these spectra  are exhibited in Fig.~\ref{fig:spectrum_comp}.  The $ E_u(k) $ plots for HD and MHD turbulence almost overlap with each other with Kolmogorov's $k^{-5/3}$ spectrum, except that for small wavenumbers, where $E_u(k)$ for MHD turbulence is larger than its HD counterpart. Since the energy is concentrated at small wavenumbers,  we observe that $U_\mathrm{MHD} > U_\mathrm{HD}$.   
\begin{figure}%[tbhp]
	\centering
	\includegraphics[scale=0.3]{fig/Figure14.pdf}
	\caption{Plots of KE spectra $E_u(k)$ for the injection rates $\epsilon_\mathrm{inj}=0.1$ (red), $\epsilon_\mathrm{inj}= 1.0$ (green) and $\epsilon_\mathrm{inj}= 10.0$ (blue). The dashed and solid curves represent the $E_u(k)$ for MHD and HD turbulence respectively. Kolmogorov's $-5/3$ scaling (black) fits well in the inertial range for both the cases. From Verma \etal~\cite{Verma:PP2020}.  Reproduced with permission from AIP.}
	\label{fig:spectrum_comp}
\end{figure}

In contrast, in DNS of Sec.~\ref{sec:dns}, $ U $ and $ E_u(k) $ of MHD turbulence are typically smaller than the corresponding values for HD turbulence.  However, In dynamo simulations, we do observe that $ U $ of MHD turbulence could be larger than that for HD turbulence; this topic will be discussed in the next section.

Next, using the numerical data of the shell model, Verma \etal \cite{Verma:PP2020}  estimated the rms values of $({\bf u}\cdot \nabla) {\bf u}$ for HD and MHD turbulence using the formula:
\be
\la  \lvert({ \bf u}\cdot \nabla) {\bf u} \rvert  \ra 
= \left(\sum_n \lvert N_n[u,u] \rvert^2 \right)^{1/2}.
\ee
To suppress the fluctuations, averaging was performed over a large number or states.   As  listed in Table~\ref{tab:HD_MHD_shell},  $ \la  \lvert({ \bf u}\cdot \nabla) {\bf u} \rvert  \ra  $ for  MHD turbulence is suppressed compared to HD turbulence.  These results reinforce  that the nonlinearity depends critically on the phases of the Fourier modes; larger $U$ does not necessarily imply larger nonlinearity. We remark that  averaging over the small $ n $ would have been more appropriate for the estimation of $ \la  \lvert({ \bf u}\cdot \nabla) {\bf u} \rvert  \ra  $, as was done for the DNS.

Verma \etal \cite{Verma:PP2020} also computed the  average kinetic energy fluxes for HD and MHD turbulence \cite{Verma:JoT2016, Verma:book:ET}. They showed  that MHD turbulence has lower KE flux than HD turbulence  for the same $\epsilon_\mathrm{inj}$ (see Fig.~\ref{fig:flux_comp} and Table~\ref{tab:HD_MHD_shell}).  This is  consistent with the suppression of nonlinearity;  lower nonlinearity leads to lower KE flux. In addition, we also compute $ \bar{c}_{d1} $ and $ \bar{c}_{d2} $ using the values of Table~\ref{tab:HD_MHD_shell}. Clearly, $ \bar{c}_{d1} $ and $ \bar{c}_{d2} $  of MHD turbulence are lower than those for HD turbulence.


\begin{figure}%[tbhp]
	\centering
	\includegraphics[scale=0.3]{fig/Figure15.pdf}
	\caption{Plot of   $\Pi_u(k)$ for   $\epsilon_\mathrm{inj}=0.1$ (red), $\epsilon_\mathrm{inj}= 1.0$ (green) and $\epsilon_\mathrm{inj}= 10.0$ (blue). The dashed curves represent the $\Pi_u(k)$ for MHD, whereas the solid curves indicate the same for HD turbulence. From Verma \etal\cite{Verma:PP2020}.  Reproduced with permission from AIP.}
	\label{fig:flux_comp}
\end{figure}


Thus, DNS  and the shell model results illustrate that MHD turbulence has lower nonlinearity and lower energy flux.  These results demonstrate a reduction in turbulent drag in MHD turbulence.   Note, however, that in DNS, the KE for MHD turbulence is lower than HD turbulence in DNS, but it is other way round in the shell model.  

In the next section we will describe turbulent drag reduction in dynamos.


